Vanilla-Converter: A Tool for Converting Camunda 7 BPMN Models into Camunda 8 Models

As organizations prepare for the end-of-life of Camunda 7, manual migration remains complex due to fundamental differences between the two platforms. We present Vanilla-Converter, a command-line tool that facilitates the migration of BPMN models from Camunda 7 to Camunda 8. Vanilla-Converter automates the transformation process, supports a wide range of BPMN elements, and produces a transformed model and a detailed transformation log indicating automatic changes and remaining manual conversion tasks. The tool's effectiveness is demonstrated through three case studies with real industrially used Camunda 7 models, confirming its ability to convert these models into valid and executable Camunda 8 models.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> save.tex <==
The symbols used in the tables have the following meanings:
\begin{itemize}
  \item \ding{51} Supported
  \item \ding{55} Not Supported
  \item \textbf{\Circle} Not Supported Yet by Camunda 8 — for details see \href{https://docs.camunda.io/docs/8.7/components/modeler/bpmn/bpmn-coverage/}{BPMN Coverage}\cite{c8-coverage}
\end{itemize}
\hfill
\begin{minipage}[b]{0.55\textwidth}
\begin{tabular}{|p{6cm}|c|}
\hline
\textbf{Element} & \textbf{Supported} \\
\hline
Service Task         & \ding{51} \\
Send Task            & \ding{51} \\
User Task            & \ding{51} \\
Business Rule Task   & \ding{51} \\
Script Task          & \ding{55} \\
Receive Task         & \ding{51} \\
Manual Task          & \ding{51} \\
Exclusive Gateway              & \ding{51} \\
Conditional / default Flows    & \ding{51} \\
Parallel Gateway               & \ding{51} \\
Inclusive Gateway              & \ding{51} \\
Event based Gateway            & \ding{51} \\
Complex Gateway                & \textbf{\Circle} \\
Multi Instance Parallel Task Marker  & \ding{51} \\
Multi Instance Sequential Task Marker  & \ding{51} \\
Ad-Hoc Task Marker                     & \textbf{\Circle} \\
Compensation  Task Marker              & \ding{51} \\
Loop  Task Marker                      & \textbf{\Circle} \\

Embedded Subprocess    & \ding{51} \\
Call activity          & \ding{51} \\
Event subprocess       & \ding{51} \\
Transaction Subprocess & \textbf{\Circle} \\
\hline
\end{tabular}
\captionof{tabular}{Supported Elements}
\label{Tab:T1}
\end{minipage}

\begin{table}[h!]
\begin{tabular}{|l|
>{\centering\arraybackslash}p{1.2cm} |
>{\centering\arraybackslash}p{1.2cm} |
>{\centering\arraybackslash}p{2cm} |
>{\centering\arraybackslash}p{1cm} |
>{\centering\arraybackslash}p{1.6cm} |
>{\centering\arraybackslash}p{1.6cm} |
>{\centering\arraybackslash}p{1cm} |
>{\centering\arraybackslash}p{1.2cm} |}
\hline
\textbf{Type} & \multicolumn{3}{c|}{\textbf{Start}} & \multicolumn{3}{c|}{\textbf{Intermediate}} & \multicolumn{2}{c|}{\textbf{End}} \\
\hline
& Normal & Event Sub Process & Event Sub Process Non- interrupt & Catch & Boundary & Boundary Non- interrupt & Throw & Normal \\
\hline
\textbf{None}         & \ding{51} & - & - & - & - & - & - & \ding{51} \\
\textbf{Message}      & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & - \\
\textbf{Timer}        & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & - & - \\
\textbf{Conditional}  & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & - & - \\
\textbf{Link}         & - & - & - & \ding{51} & - & - & \ding{51} & - \\
\textbf{Signal}       & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
\textbf{Error}        & - & \ding{51} & - & - & \ding{51} & - & - & \ding{51} \\
\textbf{Escalation}   & - & \ding{51} & \ding{51} & - & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
\textbf{Termination}  & - & - & - & - & - & - & - & \ding{51} \\
\textbf{Compensation} & - & \ding{55} & - & - & \ding{51} & - & - & \ding{51} \\
\textbf{Cancel}       & - & - & - & - & \textbf{\Circle} & - & - & \textbf{\Circle} \\
\textbf{Multiple}     & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} &  \textbf{\Circle} \\
\textbf{Multiple Parallel} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} & \textbf{\Circle} \\
\hline
\end{tabular}
\caption{Supported Event Types}
\label{Tab:T5}
\end{table}
